Simulating the Shastry-Sutherland Ising Model using Quantum Annealing

Frustration represents an essential feature in the behavior of magnetic materials when constraints on the microscopic Hamiltonian cannot be satisfied simultaneously. This gives rise to exotic phases of matter including spin liquids, spin ices, and stripe phases. Here we demonstrate an approach to understanding the microscopic effects of frustration by computing the phases of a 468-spin Shastry-Sutherland Ising Hamiltonian using a quantum annealer. Our approach uses mean-field boundary conditions to mitigate effects of finite size and defects alongside an iterative quantum annealing protocol to simulate statistical physics. We recover all phases of the Shastry-Sutherland Ising model -- including the well-known fractional magnetization plateau -- and the static structure factor characterizing the critical behavior at these transitions. These results establish quantum annealing as an emerging method in understanding the effects of frustration on the emergence of novel phases of matter and pave the way for future comparisons with real experiments.

==> unused.tex <==

%The macroscopic properties of materials depend on the strengths and symmetries of the microscopic Hamiltonian which can be controlled by an external stimulus, such as a magnetic field, or by intrinsic disorder. Understanding and tuning the phases of matter and their transitions is at the heart of modern material science. Here we establish a quantum hardware route to understanding phases of materials by successfully computing the phases of a 500-spin Shastry-Sutherland Hamiltonian on a 2000-qubit quantum annealing chip. We employ a new approach that relies on iterative quantum annealing of a model Hamiltonian to improve computational convergence. We introduce a novel use of mean-field boundary conditions and iterative exchange perturbation to tune the effects of disorder within the chip to mimic physical disorder in real materials and to mitigate the errors from finite system size. We not only recover four distinct phases predicted by Monte Carlo---including the well-known transition to a fractional magnetization plateau---within a very small number of iterations, but also identify the critical behavior at their transitions as well as the effects from disorder.  Our results establish that quantum annealing can provide a viable and accurate description of the ground state of magnetic Hamiltonians, providing an exciting pathway to understanding data obtained from scattering experiments on real spintronic materials. 

%in magnetic materials, the phase transitions have driven advances in magnetic memories, and more recently show promise of topological quantum spintronic devices in topological quantum information science. Magnetic frustration leads to phase transitions, and fluctuations therein lead to multiple degeneracy of states spanning large Hilbert spaces.  An important feature in the behavior of magnetic materials is frustration, in which all constraints on a magnetic Hamiltonian cannot be satisfied simultaneously. This gives rise to a variety of exotic phases such as the spin liquid [\cite{}], spin ice[ \cite Felsher{}], Skyrmion lattices [\cite{}] and stripy magnetic phases found in frustrated magnetic superconductors [\cite{}]. Here we demonstrate a new approach to understanding the microscopic origin of frustration by using quantum annealing to compute the phases of a 500-spin Shastry-Sutherland Hamiltonian. Our approach relies on the novel use of mean-field boundary conditions to mitigate errors from finite system size as well as iterative simulation to improve computational convergence. We recover the four phases of the Shastry-Sutherland Ising model including the well-known transition to a fractional magnetization plateau and the static structure factor characterizing the critical behavior at these transitions. These results indicate how quantum annealing can enable a better understanding of the data microscopic origin of frustration and the emergence of novel phases of matter. We introduce a novel use of mean-field boundary conditions and iterative exchange perturbation to tune the effects of disorder within the chip to mimic physical disorder in real materials and to mitigate the errors from finite system size. We not only recover four distinct phases predicted by Monte Carlo---including the well-known transition to a fractional magnetization plateau---within a very small number of iterations, but also identify the critical behavior at their transitions as well as the effects from disorder.  Our results establish that quantum annealing can provide a viable and accurate description of the ground state of magnetic Hamiltonians, providing an exciting pathway to understanding data obtained from scattering experiments on real spintronic materials. 
%Examples of these phases are found in several real materials, for example the Kagome spin liquid physics in Herbertsmithite[\cite Han{}] and Spin Ice in DyTiO3, attracting a large amount of bulk thermodynamic [\cite {QSL Rev Mod Phys Nussinov}] and scattering data [\cite {Han, others}]. The search for canonical systems complying with the geometrically frustrated lattices is complicated by the presence of inherent intrinsic defects in the real material systems, leading to non-ideal ground states with broadened phase transitions and making their theoretical understanding and computational modelling even more difficult.


%%>> Motivate study of materials simulation using quantum computing
%The advent of quantum computing has expanded modeling and simulation to include a variety of quantum computing technologies and a growing number of quantum computational methods \cite{RevModPhys.86.153, cao2019quantum}. These approaches to understanding the structural and dynamical properties of complex materials may soon surpass conventional methods \cite{arute2019quantum}, amongst an ongoing debate about how to obtain sufficient accuracy and reliability for such demonstrations. For example, recent simulations of glassy and topological spin phases using quantum annealers have validated the potential to study realistic material systems \cite{king_observation_2018,harris_phase_2018}.
%\par 
%%>> Setup up problem statement as development of QEMC and MF BC techniques for materials simulation
%Within the context of quantum annealing, quantum evolution Monte Carlo (QEMC) methods have emerged recently as an alternative for recording the low-energy manifold of states represented by a model Hamiltonian. The conventional forward annealing (FA) method relies on adiabatic evolution to prepare low-energy separable quantum states but due to various phenomena, such as system freeze-out and relaxation, practical performance is often limited \cite{amin_searching_2015,marshall_power_2019}. By contrast, QEMC leverages the advanced programmability of quantum annealers to iteratively resample a well-defined ensemble of initialized quantum states \cite{king_observation_2018,harris_phase_2018}. A single iteration relies on reverse annealing, which slowly ramps up a weak transverse field to the underlying Ising Hamiltonian, before reversing the process and measuring the prepared state. QEMC repeats this process until a desired convergence in energy is observed.
%\par 
%%>> Describe approach taken 
%Here we extend QEMC to the context of an embedded Ising spin model on a 2D, geometrically-frustrated Shastry-Sutherland (SS) lattice. The SS Ising model plays a prominent role in understanding the behavior of rare-earth tetraborides (RB$_4$), magnetic systems which exhibit a unique fractional magnetization plateau above a critical value of the applied longitudinal magnetic \cite{matas_magnetism_2010,brunt_magnetic_nodate}. A potential origin of these plateaus is due to geometrical frustration in the Ising model on an SS lattice, and it has been shown that a plateau at $1/3$ magnetization arises as the unique solution to this model above a critical longitudinal field strength \cite{dublenych_ground_2012}. Understanding this unique phase requires fair and accurate sampling of the simulated ground states across all phases of the model to ensure a correct computational characterization.
%\par 
%We characterize the bulk phase properties of the SS Ising model using QEMC to simulate the ground state manifold, which requires fair and accurate sampling across a broad range of Hamiltonian parameters. We introduce a new technique for calibrating mean-field boundary conditions of the embedded spin system that mitigates the influence of finite size effects to better approximates the bulk behavior. We then use QEMC to simulate the ground-state ensemble of the frustrated spin states and recover both the phase diagram and static structure factor for the model Hamiltonian. 


%An attractive feature of quantum annealing is the output of logical solutions, which are crucial to understand the magnetic ordering in real materials. Because of this feature we are able to verify not only the correct order parameter behavior but also the expected real-space spin motifs. As observed in Fig.~\ref{fig:phase_diagram_motifs} C) the quantum processor produces the correct real-space behavior that has been predicted in literature previously \cite{liu_magnetization_2009,dublenych_ground_2012} for this model. 

%Normally one seeks to minimize the length of chains in an embedding to improve performance. This is often treated as the only metric when evaluating the quality of an embedding, but this is not the case. Often neglected is coupler heterogeneity -- the fact that certain device couplers have different behavior from one another throughout the device operation due to typical manufacturing variation. When exploring classical magnetic phases this non-symmetric perturbation can lead to erroneous solutions. 
%Other embeddings for the Shastry-Sutherland lattice were explored but the HC embedding enabled solutions with the correct magnetic ordering.

%%
%where $z_i \in \{\pm1\}$ is the spin state of the $i$-th lattice site, $h_z$ is the applied longitudinal magnetic field, $J_1>0$ is the interaction strength between spins on square plaquettes, and $J_2>0$ is the interaction strength between spins on dimer pairs. There are three trivial phases in this model: a N\'eel antiferromagnetic (AFM) phase when $J_1 \gg J_2, h_z$, a dimer AFM phase when $J_2 \gg J_1, h_z$, and a ferromagnetic (FM) phase when $h_z \gg J_1,J_2$. However, when $J_1 \approx J_2 \approx h_z$ the system becomes geometrically frustrated and orders periodically with frequency $1/3$, forming a magnetization plateau.
%\par 
%%>> Present embedding result

%We also explored alternative embeddings but preliminary experiments indicated  the lack of symmetry in these embeddings yield poor results. 
%Fully characterizing the impact and behavior of alternative embeddings will provide invaluable information for future material simulations and is therefore a topic of future work. 


%an empirical approach to determine control parameters that elucidate the competing time-scales present in the device, and which control parameters lead to high-performance solutions. The methodology and solutions presented in this work provide new empirical insight into non-traditional annealing techniques and further demonstrate the suitability of near-term quantum annealers for applications in materials science.

%Quantum annealing has recently shown great progress in the simulation of paradigmatic models of solid-state physics but the connection to real materials and experimental techniques has been elusive.\cite{king_observation_2018,harris_phase_2018} Here we strengthen this connection, demonstrating the ability of quantum annealers to tackle problems in material science by calculating equilibrium properties of a geometrically-frustrated Ising model with closely related material realizations. Moreover we demonstrate that the obtained solutions agree quantitatively with previously predicted results and study the annealing controls and embedding considerations necessary for high performance quantum annealing.

%The variability in embedding logical problems in imperfect, sparse quantum annealers often leads to erroneous solutions due to lack of physical uniformity on-chip. Usually the quality of embeddings are determined by average chain length but here we show that chain length alone is not sufficient to describe the embedding quality. To obtain high performance out of near-term quantum annealers requires designing embeddings that utilize device inhomogeneity to reinforce the symmetries of the logical problem. This is seen in the quality of solutions obtained by the HC embedding, due to the physical-logical symmetry-enriched embedding. 

%Experimental evidence from neutron scattering suggests that the magnetic ordering is slightly longer range than typical ordering of the unit cell, which is consistent with analytic and numerical solutions to this model. Here we are able to reproduce the magnetization plateau and correct long-range spin structures observed in experiment and classical calculations by embedding and relaxing the SS lattice into the D-Wave 2000Q QPU.\cite{dublenych_ground_2012,liu_magnetization_2009,chang_magnetization_2009,huang_multi-step_2012}

%We conclude that quantum annealing is well suited for studying a broad range of materials systems using these advances in  quantum computational methods to account for boundary effects and non-zero temperatures.


%A substantial amount of work has been done in the realm of quantum information science to realize gate-model quantum computers on platforms such as superconducting transmons \cite{IBM,arute2019quantum}, as well as on trapped ions systems [\cite{Honeywell, ionQ}] and others. Some of these noisy intermediate-scale quantum (NISQ) devices have even shown promise in simulating certain material properties, each posing its own advantages and disadvantages of scalability, noise and connectivity. The state-of-the-art systems based on transmons still require a significant development to abate the effect of noise and error, while the trapped ion systems have the advantage of low noise but at the cost of limited programmability. Under these circumstances, the QA processor used herein provides immediate promise to simulate real problems.  
%We have demonstrated that quantum tunneling during an anneal allows all the pseudospins to collectively  NO we have not demonstrated whether it is tunneling, thermal activation, or something else moving us to the ground state. The system is not adiabatic in this situation.  It thermalizes to a Gibbs distribution of the quantum Hamiltonian.

%\par
%Along with expanded qubit connectivity, improvements to projective readout may allow observation of the quantum critical phases of matter, distinct from their classical counterparts, in more complex Hamiltonians---perhaps those seen in real materials. Going forward, our research indicates a pathway to simulate a variety of intriguing quantum spintronic systems using the near-term quantum hardware such as the spin ice \cite{} or the the bond frustrated Kitaev problem \cite {Kitaev, Bhaskaran, Banerjee}, while also finding Hamiltonians of real materials using quantum machine-learning approaches.

